FedL2P: Federated Learning to Personalize

Federated learning (FL) research has made progress in developing algorithms for distributed learning of global models, as well as algorithms for local personalization of those common models to the specifics of each client's local data distribution. However, different FL problems may require different personalization strategies, and it may not even be possible to define an effective one-size-fits-all personalization strategy for all clients: depending on how similar each client's optimal predictor is to that of the global model, different personalization strategies may be preferred. In this paper, we consider the federated meta-learning problem of learning personalization strategies. Specifically, we consider meta-nets that induce the batch-norm and learning rate parameters for each client given local data statistics. By learning these meta-nets through FL, we allow the whole FL network to collaborate in learning a customized personalization strategy for each client. Empirical results show that this framework improves on a range of standard hand-crafted personalization baselines in both label and feature shift situations.

==> algorithms/hypergrad.tex <==
% \begin{wrapfigure}[13]{L}{0.48\textwidth}
% \begin{minipage}{0.48\textwidth}
% \begin{algorithm}[H]
    
%     \caption{\small{Hypergradient}} \label{algo:hypergrad}
%     \vspace{-0.4em}
%     \begin{flushleft}
%     \textbf{Input:} \footnotesize{Validation Loss $\mathcal{L}_V$ and training Loss $\mathcal{L}_T$. Learning rate $\psi$ and no. of iterations $Q$.
%     Fixed point $(\lambda^{'}, \theta^*(\lambda^{'}))$}.
%     \end{flushleft}
%     \begin{algorithmic}[1]
%     \STATE $p = v = \partial_{\theta} \mathcal{L}_V |_{(\lambda^{'}, \theta^*(\lambda^{'}))}$
%     \FOR{iteration $1,\hdots,Q$}
%         \STATE $v \leftarrow v - \psi \: v \: \partial^2_{\theta^*}\mathcal{L}_T$
%         \STATE $p \leftarrow p + v$
%     \ENDFOR
%     \end{algorithmic}
    
%     \textbf{Output: $\partial_\lambda \mathcal{L}_{V} |_{(\lambda^{'}, \theta^*(\lambda^{'}))} - p \: \partial_{\lambda\theta} \mathcal{L}_T |_{(\lambda^{'}, \theta^*(\lambda^{'}))}$} 
% \end{algorithm}
% \end{minipage}
% \end{wrapfigure}

==> rebuttal_global_response.tex <==
\input{tables/commands.tex}

\begin{figure}[h]
\renewcommand\thefigure{R1}
% \centering
\includegraphics[trim=0 0pt 0 0pt, clip,width=\columnwidth]{hp/commands_250_BNNet_LRNet_e5.pdf}
\caption{Response to Reviewer wFN9 Q3.4 and Reviewer Jjav Q4.4. Locality, spread, and skewness of \method{}'s learned hyperparameters, $\boldsymbol{\beta}$ and $\boldsymbol{\eta}$, of different layers across clients and the model's sparsity of all clients for Speech Commands ($e=5$) on \textit{seen} pool of clients.}
\label{fig:hp_commands}
\end{figure}

\input{tables/cifar_extended_extended.tex}




==> tables/cifar_extended_extended.tex <==
% \begin{wrapfigure}{L}{0.48\textwidth}
% \vspace{-2.2em}
% \begin{minipage}[t]{0.48\textwidth}
\begin{table}[h]
\centering
\caption{\method{} complements existing FL methods by improving on the finetuning process. Experiments on CIFAR10 ($e=15$).}
\begin{scriptsize}
\resizebox{1.0\textwidth}{!}{\begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{|cccc|c|}
\hline
  \multicolumn{1}{|c|}{\textbf{$\boldsymbol{\alpha}$}} &
\multicolumn{1}{|c|}{\textbf{Approach}} & \multicolumn{1}{c|}{\textbf{+FT (BN C)}} & \textbf{+\method{}} & \textbf{Gain} \\ \hline
% \multicolumn{3}{|c|}{$\boldsymbol{\alpha}=1000$ ($\downarrow$ heterogeneity)} \\ \hline
\multicolumn{1}{|c|}{\textbf{1000}} &
\multicolumn{1}{|c|}{FedAvg} & \multicolumn{1}{c|}{63.04±0.02} & 65.13±0.02 & +2.09 \\ 
\multicolumn{1}{|c|}{\tiny{($\downarrow$ heterogeneity)}} &
\multicolumn{1}{|c|}{PerFedAvg(HF)} & \multicolumn{1}{c|}{34.58±0.13} & 47.58±0.01 & +13.00 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{FedBABU} & \multicolumn{1}{c|}{65.00±0.07} & 66.49±0.03 & +1.49 \\ \hline

% \multicolumn{3}{|c|}{$\boldsymbol{\alpha}=1.0$} \\ \hline
\multicolumn{1}{|c|}{\textbf{1.0}} &
\multicolumn{1}{|c|}{FedAvg} & \multicolumn{1}{c|}{61.42±0.13} & 65.76±0.31 & +4.34 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{PerFedAvg(HF)} & \multicolumn{1}{c|}{44.85±0.28} & 50.2±1.26 & +5.35 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{FedBABU} & \multicolumn{1}{c|}{68.92±0.11} & 70.71±0.28 & +1.79 \\ \hline
% \multicolumn{3}{|c|}{$\boldsymbol{\alpha}=0.5$} \\ \hline
\multicolumn{1}{|c|}{\textbf{0.5}} &
\multicolumn{1}{|c|}{FedAvg} & \multicolumn{1}{c|}{62.34±0.14} & 68.45±0.5 & +6.11 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{PerFedAvg(HF)} & \multicolumn{1}{c|}{52.43±0.16} & 55.05±0.53 & +2.62 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{FedBABU} & \multicolumn{1}{c|}{72.26±0.1} & 72.87±0.42 & +0.61 \\ \hline
% \multicolumn{3}{|c|}{$\boldsymbol{\alpha}=0.1$ ($\uparrow$ heterogeneity)} \\ \hline
\multicolumn{1}{|c|}{\textbf{0.1}} &
\multicolumn{1}{|c|}{FedAvg} & \multicolumn{1}{c|}{79.15±0.07} & 80.28±0.07 & +1.13 \\ 
\multicolumn{1}{|c|}{\tiny{($\uparrow$ heterogeneity)}} &
\multicolumn{1}{|c|}{PerFedAvg(HF)} & \multicolumn{1}{c|}{77.31±0.05} & 77.68±0.13 & +0.37 \\ 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{|c|}{FedBABU} & \multicolumn{1}{c|}{79.50±0.08} & 79.58±0.04 & +0.08 \\ \hline
\end{tabular}
\end{center}
\end{minipage}
}
\end{scriptsize}
\label{tab:extend_cifar}
\vspace{-1.0em}
\end{table}
% \end{wraptable}
% \end{minipage}
% \end{wrapfigure}

==> tables/hp.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[!t]
% \label{tab:hp}
% \centering
% \caption{\hl{IMPORTANT: DO WE NEED THIS TABLE? Shows the mean and SD of mean of $\boldsymbol{\beta}$, mean of $\boldsymbol{\eta}$, and sparsity across all clients}}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} &
%   \textbf{Epochs (e)} &
%   \textbf{$\boldsymbol{\alpha}$} &
%   \textbf{Mean($\boldsymbol{\beta}$)} &
%   \textbf{Mean($\boldsymbol{\eta}$)} &
%   \textbf{Sparsity} \\ \hline
% \multirow{2}{*}{\textbf{CIFAR10}} &
%   5 &
%   \begin{tabular}[c]{@{}c@{}}1000\\ 1.0\\ 0.5\\ 0.1\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.15±2e-3\\ 0.0±0.0\\ 0.0±0.0\\ 0.0±0.0\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}2e-4±3e-6\\ 9e-4±4e-6\\ 2e-3±9e-5\\ 2e-4±1e-5\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.31±3e-3\\ 0.13±6e-3\\ 0.55±0.02\\ 0.95±1e-3\end{tabular} \\ \cline{2-6} 
%  &
%   15 &
%   \begin{tabular}[c]{@{}c@{}}1000\\ 1.0\\ 0.5\\ 0.1\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.0±0.0\\ 0.0±0.0\\ 0.0±0.0\\ 0.0±0.0\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.0±0.0\\ 7e-4±1e-5\\ 4e-4±0.0\\ 1e-4±1e-6\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}1.0±0.0\\ 0.69±1e-3\\ 0.27±0.01\\ 0.94±0.01\end{tabular} \\ \hline
% \textbf{CIFAR-10C} &
%   15 &
%   \begin{tabular}[c]{@{}c@{}}1000\\ 1.0\\ 0.5\\ 0.1\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.7±0.0\\ 0.3±0.0\\ 0.22±3e-3\\ 0.0±0.0\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}2e-3±3e-5\\ 1e-3±0.0\\ 3e-4±0.0\\ 1e-4±1e-6\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.29±4e-3\\ 0.16±0.0\\ 0.38±0.01\\ 0.66±0.07\end{tabular} \\ \hline
% \textbf{Caltech-10} &
%   15 &
%   1000 &
%   0.45±7e-4 &
%   8e-3±0.0 &
%   0.0±0.0 \\ \hline
% \textbf{DomainNet} &
%   15 &
%   \begin{tabular}[c]{@{}c@{}}1000\\ 1.0\\ 0.5\\ 0.1\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.30±1e-3\\ 0.06±2e-3\\ 0.56±1e-3\\ 0.27±2e-3\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}6e-3±0.0\\ 4e-3±9e-6\\ 1e-2±0.0\\ 3e-2±2e-5\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.0±0.0\\ 0.33±1e-3\\ 0.0±0.0\\ 0.03±0.0\end{tabular} \\ \hline
% \end{tabular}
% \end{table*}
